Approximate Bipartite $b$-Matching using Multiplicative Auction

Given a bipartite graph $G(V= (A \cup B),E)$ with $n$ vertices and $m$ edges and a function $b \colon V \to \mathbb{Z}_+$, a $b$-matching is a subset of edges such that every vertex $v \in V$ is incident to at most $b(v)$ edges in the subset. When we are also given edge weights, the Max Weight $b$-Matching problem is to find a $b$-matching of maximum weight, which is a fundamental combinatorial optimization problem with many applications. Extending on the recent work of Zheng and Henzinger (IPCO, 2023) on standard bipartite matching problems, we develop a simple auction algorithm to approximately solve Max Weight $b$-Matching. Specifically, we present a multiplicative auction algorithm that gives a $(1 - \varepsilon)$-approximation in $O(m \varepsilon^{-1} \log \varepsilon^{-1} \log \beta)$ worst case time, where $\beta$ the maximum $b$-value. Although this is a $\log \beta$ factor greater than the current best approximation algorithm by Huang and Pettie (Algorithmica, 2022), it is considerably simpler to present, analyze, and implement.

==> sections/bmatching.tex <==
\section{Extension to $b$-Matching} \label{sec:bMatching}

In this section we extend the auction approach to
\maxwbm{}, whose LP-Relaxation \cref{lp:bmatching_primal} (i.e.~the primal) and dual \cref{lp:bmatching_dual} are given by

\vspace{-3ex} 
\leqnomode
\noindent\begin{minipage}[t]{.47\linewidth}
    \begin{maxi*}
        {}{\sum_{(i, j) \in E} w(i,j) x(i,j)}{}{}{} %\label{lp:bmatching_primal}
        \label[lp]{lp:bmatching_primal} \tag{$\mathsf{P_2}$}
        \addConstraint{\sum_{j \in N(i)} x(i,j)}{\leq \bv[i]}{\; \forall i \in A}
        \addConstraint{\sum_{i \in N(j)} x(i,j)}{\leq \bv[j]}{\; \forall j \in B} 
        \addConstraint{0 \leq x(i,j)}{\leq 1}{\; \forall \lrp{i,j} \in E}.
    \end{maxi*}
\end{minipage}%
\begin{minipage}[t]{.6\linewidth}
    \begin{mini*}
        {}{\sum_{i \in A} \bv[i] \pi(i) + \sum_{j \in B} \bv[j] p(j) + \sum_{(i,j) \in E} z(i, j)}{}{}{} %\label{lp:bmatching_dual}
        \label[lp]{lp:bmatching_dual} \tag{$\mathsf{D_2}$}
        \addConstraint{\pi(i) + p(j) + z(i, j)}{\geq w(i,j)}{\; \forall \lrp{i, j} \in E}
        \addConstraint{z(i, j)}{ \geq 0}{\; \forall \lrp{i,j} \in E}
        \addConstraint{\pi(i),\;p(j)}{ \geq 0}{\; \forall i \in A, j\in B}.
    \end{mini*}
\end{minipage}
\reqnomode

\vspace{1em}
In addition to those stated in \cref{lem:comp_slack}, the complementary slackness conditions for the \maxwbm{} problem include  
\begin{align}
    \sum_{j \in N(i)} x^{\ast}(i, j) < \bv[i] \implies \pi^{\ast}(i) = 0 \quad &\forall i \in A %\\
    \label{eq:bmatching_comp_slack_profit}\\
    \sum_{i \in N(j)} x^{\ast}(i, j) < \bv[j] \implies p^{\ast}(j) = 0 \quad &\forall j \in B.
    \label{eq:bmatching_comp_slack_price}
\end{align} 
for optimal primal and dual solutions $x^{\ast}, \pi^{\ast}, p^{\ast}$.
That is, any unsaturated vertices have a dual value of zero, which motivates a slightly different formulation of $\varepsilon$-happiness. 
\begin{definition}[$b$-Matching $\varepsilon$-Happiness]
    \label{def:epsilon_happy_edge_bmatching}
    For a set of matched edges $F$ and prices $p$, 
    an edge $\lrp{i, j} \in F$ is $\varepsilon$-happy if 
    \begin{equation*}
        w(i,j) - p(j) \geq \max_{k \in N(i) \sm F(i)} \lrc{w(i,k) - p(k)} - \varepsilon
    \end{equation*}
    where $w(i,j) - p(j) \geq 0$ and the profit is given by $\pi(i) \coloneqq \max \lrc{0, \max_{k \in N(i) \sm F(i)} \lrc{w(i,k) - p(k)} - \varepsilon}$. 
    A bidder $i$ is $\varepsilon$-happy if all edges $\lrp{i, j} \in F$ are $\varepsilon$-happy and either
    \textbf{\textsf{(1)}} $i$ is saturated by $F$ and $\max_{k \in N(i) \sm F(i)} \lrc{w(i,k) - p(k)} - \varepsilon \geq 0$ or 
    \textbf{\textsf{(2)}} $i$ is unsaturated by $F$  and $\max_{k \in N(i) \sm F(i)} \lrc{w(i,k) - p(k)} - \varepsilon \leq 0$.
    %%% For two columns %%%
    %\begin{align*}
    %    w(i,j) - p(j) &\geq  0 = \pi(i) \\ 
    %    &\geq \max_{k \in N(i) \sm F(i)} \lrc{w(i,k) - p(k)} - \varepsilon. 
    %\end{align*}
\end{definition}
 
\begin{comment}  
    \begin{definition}[$b$-Matching $\varepsilon$-Happiness]
    \label{def:epsilon_happy_edge_bmatching}
    For a set of edges $F$ and price function $p$, 
    a bidder $i$ is $\varepsilon$-happy if 
    it satisfies one of the following: \textbf{(1)} $i$ is saturated by $F$ and all edges $\lrp{i, j} \in F$ satisfy 
    \begin{equation*}
        w(i,j) - p(j) \geq \max_{k \in N(i) \sm F(i)} \lrc{w(i,k) - p(k)} - \varepsilon = \pi(i) 
    \end{equation*}
    or \textbf{(2)} $i$ is unsaturated by $F$, and all edges $\lrp{i, j} \in F$ satisfy 
    \begin{equation*}
        w(i,j) - p(j) \geq \pi(i) = 0 \geq \max_{k \in N(i) \sm F(i)} \lrc{w(i,k) - p(k)} - \varepsilon. 
    \end{equation*}
    %%% For two columns %%%
    %\begin{align*}
    %    w(i,j) - p(j) &\geq  0 = \pi(i) \\ 
    %    &\geq \max_{k \in N(i) \sm F(i)} \lrc{w(i,k) - p(k)} - \varepsilon. 
    %\end{align*}
\end{definition}

    \begin{itemize}
        \item it is saturated by $F$ and all edges $\lrp{i, j} \in F$ satisfy 
        \begin{equation*}
            w(i,j) - p(j) \geq \max_{k \in N(i) \sm F(i)} \lrc{w(i,k) - p(k)} - \varepsilon = \pi(i). 
        \end{equation*}
        \item it is unsaturated by $F$ and all edges $\lrp{i, j} \in F$ satisfy 
        \begin{equation*}
            w(i,j) - p(j) \geq \pi(i) = 0 \geq \max_{k \in N(i) \sm F(i)} \lrc{w(i,k) - p(k)} - \varepsilon. 
        \end{equation*}
    \end{itemize} 
\end{comment}  

If $F$ is $\varepsilon$-happy, note that it automatically satisfies \cref{eq:bmatching_comp_slack_profit}. 
If $F,p$ additionally satisfy \cref{eq:bmatching_comp_slack_price}, then the weight of $F$ falls within an additive loss of the optimal weight. 
The proof of the following theorem is very similar to the proof of \cref{thm:additive_loss_bfactor} and is included in
in \cref{subsec:proof_additive_loss_bmatching}.% due to space constraints. 
 
\begin{theorem}
    Let $F, p$ be some feasible \bmatching{} and prices, respectively, such that $F$ is $\varepsilon$-happy 
    and $F, p$ satisfy \cref{eq:bmatching_comp_slack_price}. Then
    \begin{equation*} 
        w(F) \geq w(F^{\ast}) - \varepsilon \abs{F^{\ast}} %\geq w(F^{\ast}) - \varepsilon \min \lrc{b(A), b(B)}
    \end{equation*}
    where $F^{\ast}$ is an optimal \bmatching{} and $\abs{F^{\ast}} \leq \min \lrc{b(A), b(B)}$. 
    \label{thm:additive_loss_bmatching}
\end{theorem}

\begin{corollary}
    Suppose that edge weights are integral. 
    If $\varepsilon < \frac{1}{\min \lrc{b(A), b(B)}}$ and $F, p$ are some feasible \bmatching{} and prices, respectively, such that $F$ is $\varepsilon$-happy 
    and $F, p$ satisfy \cref{eq:bmatching_comp_slack_price}, then $F$ is optimal. 
    \label{cor:bmatching_integral}
\end{corollary}
\begin{corollary}
    Suppose that edge weights are integral (or more generally given by $w \colon E \to \lrc{0} \cup \R_{\geq 1}$). 
    Let $F, p$ be some feasible \bmatching{} and prices, respectively, such that $F$ is $\varepsilon$-happy 
    and $F, p$ satisfy \cref{eq:bmatching_comp_slack_price}.
    Then $F$ is a $\lrp{1 - \varepsilon}$-approximation of the optimal solution. 
    \label{cor:bmatching_const_factor_approx}
\end{corollary}
\begin{proof}
    By \cref{thm:additive_loss_bmatching}
    \begin{equation*}
        w(F) \geq w(F^{\ast}) - \varepsilon \abs{F^{\ast}} \geq \lrp{1 - \varepsilon} w(F^{\ast}),
    \end{equation*}
    where $\abs{F^{\ast}} \leq w(F^{\ast})$ follows since $F^{\ast}$ does not need to contain any edges of weight $0$ and hence all the edges in $F^{\ast}$ have weight at least $1$. 
\end{proof}

\subsection{The Algorithm} \label{subsec:alg_bmatching}
Similar to \cref{sec:auction}, it is again useful to consider the idea of each object having a set of copies and 
a notion of strong $\varepsilon$-happiness in place of $\varepsilon$-happiness. 
\begin{definition}[$b$-Matching Strong $\varepsilon$-Happiness]
    \label{def:strong_epsilon_happy_edge_bmatching}
    For a set of edges $F$ and internal prices for each object copy, an edge $\lrp{i, j} \in F$, where $i$ is assigned 
    to $c \in M(j)$,
    %an assignment of a bidder $i$ to some object copy $c$, where $c \in M(j)$, 
    is strongly $\varepsilon$-happy if it satisfies  
    \begin{equation*}
        w(i,j) - p_j(c) \geq \max_{k \in N(i) \sm F(i), \; l \in M(k)} \lrc{w(i,k) - p_{k}(l)} - \varepsilon
    \end{equation*}
    where $w(i,j) - p_j(c) \geq 0$ and the profit is given by
    $\pi(i) \coloneqq \max \{0, \max_{k \in N(i) \sm F(i), \; l \in M(k)} \lrc{w(i,k) - p_{k}(l)} - \varepsilon\}$. 
    A bidder $i$ is strongly $\varepsilon$-happy if all edges $\lrp{i, j} \in F$ are strongly $\varepsilon$-happy and
    \textbf{\textsf{(1)}} $i$ is saturated by $F$ and $\max_{k \in N(i) \sm F(i), \; l \in M(k)} \lrc{w(i,k) - p_{k}(l)} - \varepsilon \geq 0$
    or
    \textbf{\textsf{(2)}} $i$ is unsaturated by $F$ and  
    $\max_{k \in N(i) \sm F(i), \; l \in M(k)} \lrc{w(i,k) - p_{k}(l)} - \varepsilon \leq 0$. 
\end{definition}

==> sections/multi-pseudocode-v2.tex <==
\usepackage{multicol}
\begin{algorithm*}[!t] 
    \caption{Multiplicative Auction} \label{alg:mult_auction_bmatching}
    \begin{multicols}{2}
    \begin{algorithmic}[1]
        \AlgIn $G = \lrp{V = \lrp{ A \cup B}, E}$, weights $\tilde{w} \colon E \to \R_{\geq 0}$, vertex capacities \bfunc{}, 
        and $\varepsilon \in (0, \frac{1}{2})$
        \AlgOut A set of edges $F$ such that $F$ is a strongly $\varepsilon$-happy \bmatching{}

        \State $I \gets A$ \Comment{Bidders that are not strongly $\varepsilon$-happy}
        \State $F \gets \emptyset$ \Comment{Matched edges}
        \State $r_i \gets 0, Q_i \gets \emptyset$ for all $i \in A$ \Comment{Queue for each bidder $i$}
        %\State $Q_i \gets \emptyset$ for all $i \in A$ \Comment{Queue for each bidder $i$}
        \State $L_r \gets \emptyset$ for all $r$ from $s_{\max}$ to $-s_{\min}$ 
        \For{$j \in B$}
            \State $M(j) \gets \lrc{c_1, \ldots, c_{b(j)}}$,  $p_j(c) \gets 0$ for all $c \in M(j)$
            %\State $p(j) \gets 0$
        \EndFor
        \For{$(i, j) \in E$} \label{line:gbs_start}
        \Comment{\textbf{Initialization Phase}}
            \State $r_{ij} \gets \textsc{iLog}(\tilde{w}(i, j))$, $r_i \gets \max \{r_i, r_{ij}\}$ 
            %\State $r_i \gets \max \{r_i, r_{ij}\}$
            \For{$r$ from $r_{ij}$ to $r_{ij} - s_{\min}$}
                $L_r \gets L_r \cup (r, (i, j))$
            \EndFor
        \EndFor \label{line:gbs_end}
        \For{$r$ from $s_{\max}$ to $-s_{\min}$} \label{line:qstart}
            \For{$(r, (i, j)) \in L_r$}
                $Q_i$.push($(r, (i, j))$)
            \EndFor
        \EndFor \label{line:qend}
        \While{$I \neq \emptyset$}
        \Comment{\textbf{Auction Phase}}
            \State Choose some $i \in I$ %\Comment{$\abs{\calI} = 1$ for serial, $\abs{\calI} > 1$ for parallel}
            \State $\Call{AssignAndBid}{i}$
        \EndWhile
        \State \Return $F$
 
        \Procedure{AssignAndBid}{$i$} %, $F$, $I$}
            %\LComment{Matching Phase}
            \State $T \gets \emptyset$ \Comment{Temporary List}%\gets \lrc{\lrv{j_{\ell}, c_{\ell}} \colon \lrv{j_{\ell}, c_{\ell}} \text{ are object and object copy pairs } i \text{ is already assigned to in } F}$
            \While{$Q_i \neq \emptyset$ and $\abs{F(i)} < \bv[i]$}
                \State $\lrp{r, (i, j)} \gets Q_i$.pop(), $r_i \gets r$ 
                \If{$j \in F(i)$}
                    \State Let $c \in M(j)$ be the object copy $i$ is assigned to 
                    \If{$\lrv{j, c} \notin T$ and $\tilde{w}(i, j) - p_j(c) \geq (1 + \varepsilon)^r$}
                        $T \gets T \cup \lrc{\lrv{j, c}}$
                    \EndIf
                \Else{}
                    \State $c \gets \argmin_{c^\prime \in M(j)} {p_j(c^\prime)}$ \label{line:obj_copy}
                    \If{$\tilde{w}(i, j) - p_j(c) \geq (1 + \varepsilon)^r$}
                        \Call{Match}{$i, \lrv{j, c}$}, $T \gets T \cup \{ \lrv{j, c} \}$
                    \EndIf
                \EndIf
            \EndWhile
            %\LComment{Price Update Phase}
            \For{$\lrv{j, c} \in T$}
                \State $\gamma_{i, c} \gets \tilde{w}(i, j) - p_j(c) - (1-\varepsilon)(1+\varepsilon)^{r_i+1}$
                \Comment{Bid value}
                \State $p_j(c) \gets p_j(c) + \gamma_{i, c}$ \Comment{Price update} \label{line:price_update}
            \EndFor
            \State $I \gets I \sm \lrc{i}$ \Comment{$i$ becomes strongly $\varepsilon$-happy}
        \EndProcedure

        \Procedure{Match}{$i, \lrv{j, c}$}
            \If{$c$ is already assigned to another bidder $y \neq i$} 
                \State $F \gets F \sm \lrc{\lrp{y, j}}$  \Comment{Remove previous edge}
                \If{$Q_y \neq \emptyset$}
                    $I \gets I \cup \lrc{y}$
                \EndIf
            \EndIf
            \State $F \gets F \cup \{ (i, j) \}$
            \Comment{$i$ gets matched to $j$ and assigned to $c$}
        \EndProcedure
    \end{algorithmic}
    \end{multicols}
\end{algorithm*}

